dacl10k: Benchmark for Semantic Bridge Damage Segmentation

Reliably identifying reinforced concrete defects (RCDs)plays a crucial role in assessing the structural integrity, traffic safety, and long-term durability of concrete bridges, which represent the most common bridge type worldwide. Nevertheless, available datasets for the recognition of RCDs are small in terms of size and class variety, which questions their usability in real-world scenarios and their role as a benchmark. Our contribution to this problem is "dacl10k", an exceptionally diverse RCD dataset for multi-label semantic segmentation comprising 9,920 images deriving from real-world bridge inspections. dacl10k distinguishes 12 damage classes as well as 6 bridge components that play a key role in the building assessment and recommending actions, such as restoration works, traffic load limitations or bridge closures. In addition, we examine baseline models for dacl10k which are subsequently evaluated. The best model achieves a mean intersection-over-union of 0.42 on the test set. dacl10k, along with our baselines, will be openly accessible to researchers and practitioners, representing the currently biggest dataset regarding number of images and class diversity for semantic segmentation in the bridge inspection domain.

==> SupplMat/1_ClassDefs.tex <==
\newcolumntype{J}[1]{>{\centering\arraybackslash}m{#1}}
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
\ctable[
star,
caption = {Concrete defects, their visual appearance, cause and example images with according annotation.},
label = tab:ConcreteDefects,
pos = ht,
width=\textwidth,
doinside=\footnotesize,
captionskip=0.6ex,
]
{p{0.092\textwidth}m{0.25\textwidth}m{0.30\textwidth}m{0.269\textwidth}}
{
	% \tnote[1]{Footnote.}
}
{\FL
Damage & Visual appearance & Cause & Example \ML
Crack
    & 
    \begin{itemize}[leftmargin=*]
        \item Elongated and narrow zigzag line
        \item Clearly darker compared to the surrounding area or black
    \end{itemize}
    & 
    \begin{itemize}[leftmargin=*]
        \item Concrete’s tensile strength is exceeded
        \item Too high bending or shearing load 
        \item Settlement of the substructure 
    \end{itemize}
    &
    \includegraphics[height=4.7cm]{SupplMat/img_SupplMat/img_ClassDefs/08857.pdf} % 08857
    \NN
    
Alligator Crack
(ACrack)
    & 
    \begin{itemize}[leftmargin=*]
        \item Many branched cracks
        \item Mostly arbitrarily orientated
        \item Usually with a small crack width (compared to \textit{Crack})
    \end{itemize}
    & 
    \begin{itemize}[leftmargin=*]
        \item Inadequate post-treatment or concrete recipe (shrinkage)
        \item Too high temperatures during hardening of the concrete
        \item Formation of expansive phases leading to a volume increase in the concrete as a result of chemical action
    \end{itemize}
    &
    \includegraphics[height=4.7cm]{SupplMat/img_SupplMat/img_ClassDefs/00521.pdf} % 00521
    \NN
       
Efflorescence
    & 
    \begin{itemize}[leftmargin=*]
        \item Mostly roundish areas of white to yellowish or reddish color
        \item Strong efflorescence can look similar to stalactites. 
        \item Often appears in weathered (\textit{Weathering}) or wet areas (\textit{WetSpot}) of the building and in combination with \textit{Crack} and/or \textit{Rust}
    \end{itemize}
    & 
    \begin{itemize}[leftmargin=*]
        \item Dissolving of salts (calcium, sodium, potassium) from the cement stone or aggregate by humidity changes or water ingress, \eg constantly running water through the building part or along its surface
        \item The salts consequently carbonate leading to the final visual appearance.
        \item Note: Water ingress can be caused by other defects imposing the draining of water, \eg, \textit{Restformwork} or damaged \textit{Drainage}. \textit{Efflorescences} are also called Calcium leaching.
    \end{itemize}
    &
    \includegraphics[height=4.7cm]{SupplMat/img_SupplMat/img_ClassDefs/02903.pdf} % 03017 01108
    \NN

Rockpocket
    & 
    \begin{itemize}[leftmargin=*]
        \item Visible coarse aggregate or punctual cavities
        \item Often in tilts of the formwork and the bottom of building parts (opposite side from which the concrete is poured into the formwork) 
    \end{itemize}
    & 
    \begin{itemize}[leftmargin=*]  
        \item Inadequate rheological properties (viscosity, yield point) of the concrete 
        \item Appears due to bad compacting after having poured the concrete into the formwork.
        Therefore, insufficient deaeration of the concrete follows causing areas in which the cement paste didn't fill the volume between the aggregate completely (\textit{Rockpocket}). 
        \item Note: Hence, the concrete cover of the reinforcement as well as the bond between the bars and the concrete is not provided or reduced. \textit{Rockpockets} are also called Honeycombing. 
    \end{itemize}
    &
 \includegraphics[height=4.7cm]{SupplMat/img_SupplMat/img_ClassDefs/05618.pdf} % Really Huge Rockpocket: 131-05_126374
    \LL
}

\ctable[
star,
caption = {Concrete defects, their visual appearance, cause and example images with according annotation.},
% label = tab:ConcreteDefects,
pos = ht,
width=\textwidth,
doinside=\footnotesize,
captionskip=0.6ex,
continued
]
{p{0.092\textwidth}m{0.25\textwidth}m{0.30\textwidth}m{0.269\textwidth}}
{
	% \tnote[1]{Footnote.}
}
{\FL
Damage & Visual appearance & Cause & Example \ML

Washouts/
Concrete corrosion
(WConccor)
    & 
    \begin{itemize}[leftmargin=*]
        \item Washouts and Concrete corrosion are indicated by a planar erosion of the concrete
        \item Note: \textit{Washouts} and \textit{Concrete corrosion} are visually hard to differ (that's why we summarized them in one class) but they are two different defect types. According to inspection standards they have to subdivided.            
    \end{itemize}
    & 
    \begin{itemize}[leftmargin=*]
        \item Washouts appear on building parts that are constantly in contact with running water leading to the erosion of the concrete, \eg, abutment walls or bridge piers in rivers.   
        \item In the interest of simplification, we describe all other forms of planar loss of concrete than \textit{Spalling} as \textit{Concrete corrosion}, \eg due to frost-thaw cycles, loss in succession to chemical attacks or abrasion (mechanical or action of acid and salt solutions). 
    \end{itemize}
    &
    \includegraphics[height=4.7cm]{SupplMat/img_SupplMat/img_ClassDefs/09317.pdf} % 09317 02682        
    \NN

Hollowareas
    & 
    \begin{itemize}[leftmargin=*]
        \item Hollow areas are not visually recognizable but their markings made with crayons (mostly yellow, red or blue) during close-up/hands-on inspections.
        \item Note: The outer edge of the marking is considered as the boundary of the according area. We annotated every chalk marking that approximately forms a closed geometric figure. Single lines were not labeled as \textit{Hollowareas} as they are often used for the marking of \textit{Cracks}.   
    \end{itemize}
    & 
    \begin{itemize}[leftmargin=*]
        \item Corrosion of the subjacent reinforcement which leads to a volume increase surrounding the reinforcement bar and detaching of the concrete area that covers the bars. 
        \item Hollowareas are usually the preliminary stage of \textit{Spallings} and \textit{Exposed Rebars}.
        \item Note: Recognizing \textit{Hollowareas} is very important as the falling concrete parts can cause severe damage. Therefore, hollow sounding areas are usually removed instantly. 
    \end{itemize}
    &
    \includegraphics[height=4.7cm]{SupplMat/img_SupplMat/img_ClassDefs/02600.pdf} % 02600
    \NN

Spalling
    & 
    \begin{itemize}[leftmargin=*]
        \item Spalled concrete area revealing the coarse aggregate
        \item Significantly rougher surface (texture) inside the \textit{Spalling} than in the surrounding surface
    \end{itemize}
    & 
    \begin{itemize}[leftmargin=*]
        \item Corrosion of the subjacent reinforcement leading to an increase in volume and consequent spalling of the concrete cover 
        \item Frost-thaw cycles of intruded water (deeper than \textit{Washouts/Concrete corrosion}) 
        \item Impact from vehicles, damaging during assembly of the building part or removal of the formwork, manufacturing faults    
    \end{itemize}
    &
    \includegraphics[height=4.7cm]{SupplMat/img_SupplMat/img_ClassDefs/07785.pdf} % 07785
    \NN

Restformwork
    & 
    \begin{itemize}[leftmargin=*]
        \item Left pieces of formwork in joints or on the structure's surface
        \item Restformwork can be made of wood and polystyrene (PS).
        \item PS is often used as a placeholder in joints during concreting.
    \end{itemize}
    & 
    \begin{itemize}[leftmargin=*]
        \item After the concrete hardening has ended, PS is often forgotten to be removed (\eg, in the joint between the abutment wall and the superstructure).
        \item Note: If \textit{Restformwork} is not removed, water may be hindered to drain which can lead to other defects (\eg \textit{Spalling}, \textit{Exposed Rebars}, \textit{Rust}).
    \end{itemize}
    &
    \includegraphics[height=4.7cm]{SupplMat/img_SupplMat/img_ClassDefs/02252.pdf} % 02252
    \LL
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ctable[
star,
caption = {General defects, their visual appearance, cause and example images with according annotation.},
label = tab:GeneralDefects,
pos = ht,
width=\textwidth,
doinside=\footnotesize,
captionskip=0.6ex,
]
{p{0.092\textwidth}m{0.25\textwidth}m{0.30\textwidth}m{0.269\textwidth}}
{
	% \tnote[1]{Footnote.}
}
{ \FL
Damage & Visual appearance & Cause & Example \ML
Wetspot
    & 
    \begin{itemize}[leftmargin=*]
        \item Wet/darker mirroring area
    \end{itemize}
    & 
    \begin{itemize}[leftmargin=*]
        \item Water is hindered to drain (through \textit{Restformwork}) or can't drain properly due to damaged \textit{Drainage}, leaky \textit{Expansion Joints}, \textit{Joint Tapes}, or \textit{Cracks} in the bridge deck.
        \item Note: There may be temporary \textit{Wetspots} due to recent rainfall which can be irrelevant for the bridge assessment. But, they may also indicate that the according area has to be observed in detail due to the greater exposition. In addition, the water can carry deicing salt (on road bridges). Usually, those areas are chosen to execute further investigations such as drill tests in order to determine the carbonation depth or chloride content.    
    \end{itemize}
    &
    \includegraphics[height=4.7cm]{SupplMat/img_SupplMat/img_ClassDefs/04439.pdf} % 04439
    \NN
    
Rust
    & 
    \begin{itemize}[leftmargin=*]
        \item Reddish to brownish area
        \item Often appears on concrete surfaces and metallic objects 
    \end{itemize}
    & 
    \begin{itemize}[leftmargin=*]
        \item Rust on the concrete surface originates from oxidation of the subjacent or neighboring reinforcement bars, or neighboring metallic building parts. The bars can corrode as a result of loss of the alkaline protective layer provided by "un-carbonated" concrete (pH value $>$ 9.5). If the pH value drops due to the further carbonation of the concrete (pH value $\leq$ 9.5), which is unavoidable over time, the reinforcement can oxidize.
        \item The carbonation is accelerated by \textit{Cracks} \textit{Rockpockets} and porous concrete because of faster intruding of water and carbon into the building part. In addition, the oxidation is intensified by deicing salts which is one of the most severe problems on road bridges. 
        % \item Regarding metallic objects the corrosion originates from the object itself. 
    \end{itemize}
    &
    \includegraphics[height=4.7cm]{SupplMat/img_SupplMat/img_ClassDefs/00454.pdf} % 00454
    \NN

Graffiti
    & 
    \begin{itemize}[leftmargin=*]
        \item All kinds of paintings on concrete and objects apart from defect markings
    \end{itemize}
    & 

    &
    \includegraphics[height=4.7cm]{SupplMat/img_SupplMat/img_ClassDefs/05516.pdf} % 05516
    \NN

Weathering
    & 
    \begin{itemize}[leftmargin=*]
        \item Summarizes all kinds of weathering on the structure (\eg smut, dirt, debris) and Vegetation (\eg plait, algae, moss, grass, plants).
        \item Weathering leads to a darker or greenish concrete surface compared to the rest of the surface. 
    \end{itemize}
    & 
    \begin{itemize}[leftmargin=*]
        \item Directly weathered areas
        \item Result of \textit{Wetspot}
        \item Note: \textit{Weathering} itself is not a severe defect. The main issue is that it can obscure other defects (\eg corroded reinforcement or cracks). \textit{Weathering} is also called Contamination.
    \end{itemize}
    &
    \includegraphics[height=4.7cm]{SupplMat/img_SupplMat/img_ClassDefs/05320.pdf} % 05320 (WeatheredConcrete) 02659 (WeatheredUeko)
    \LL
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ctable[
star,
caption = {Objects, their visual appearance, functionality including their role for the bridge assessment and example images with according annotation.},
label = tab:Objects,
pos = ht,
width=\textwidth,
doinside=\footnotesize,
captionskip=0.6ex,
]
{p{0.092\textwidth}m{0.25\textwidth}m{0.30\textwidth}m{0.269\textwidth}}
{
	% \tnote[1]{Footnote.}
}
{ \FL
Object & Visual appearance & Functionality & Example \ML
Exposed Rebars 
    & 
    \begin{itemize}[leftmargin=*]
        \item Exposed Reinforcement (non-prestressed and prestressed) and cladding tubes of tendons
        \item Often appears in combination with \textit{Spalling} or \textit{Rockpocket}, and \textit{Rust}
    \end{itemize}
    & 
    \begin{itemize}[leftmargin=*]
        \item In reinforced concrete structures, the reinforcement's task concerning the load transfer is to absorb the tensile forces.
        \item \textit{Exposed Rebars} occur due to insufficient concrete cover or corrosion and the consequent \textit{Spalling} of the concrete cover.
        \item The reduction of the reinforcement's cross section due to \textit{Rust} significantly influences the structural integrity of the according building.
    \end{itemize}
    &
    \includegraphics[height=4.7cm]{SupplMat/img_SupplMat/img_ClassDefs/09360.pdf} % 09360
    \NN
    
Bearing
    & 
    \begin{itemize}[leftmargin=*]
        \item  All kinds of bearings, such as rocker-, elastomer- or spherical-bearings
    \end{itemize}
    & 
    \begin{itemize}[leftmargin=*]
        \item Bearings transfer the load from the superstructure to the substructure.
        \item Note: Bearings can show \textit{Rust} and \textit{Cracks} as well as deformation due to settlements in the abutments, overloading or creeping of the bridge. 
        The deformation or damaging of bearings can result in load redistribution which is not considered in the structural design of the bridge. 
    \end{itemize}
    &
    \includegraphics[height=4.7cm]{SupplMat/img_SupplMat/img_ClassDefs/03647.pdf} % 03647
    \NN

Expansion Joint \linebreak
(EJoint)
    & 
    \begin{itemize}[leftmargin=*]
        \item Located at the beginning and end of the bridge
        \item Assembled cross to the longitudinal bridge axis
    \end{itemize}
    & 
    \begin{itemize}[leftmargin=*]
        \item \textit{Expansion Joints} compensate the thermal longitudinal expansion of the bridge deck and superstructure.
        \item Note: Mostly, \textit{Expansion Joints} are corroded (\textit{Rust}) and weathered (\textit{Weathering}) which hinders their ability to compensate the enlargements due to changes in temperature.
    \end{itemize}
    &
    \includegraphics[height=4.7cm]{SupplMat/img_SupplMat/img_ClassDefs/06160.pdf} % 06160
    \LL
}

\ctable[
star,
caption = {Object classes, their visual appearance, functionality including their role for the bridge assessment and example images with according annotation.},
% label = tab:Objects,
pos = ht,
width=\textwidth,
doinside=\footnotesize,
captionskip=0.6ex,
continued
]
{p{0.092\textwidth}m{0.25\textwidth}m{0.30\textwidth}m{0.269\textwidth}}
{
	% \tnote[1]{Footnote.}
}
{ \FL
Object & Visual appearance & Functionality & Example \ML
Drainage
    & 
    \begin{itemize}[leftmargin=*]
        \item  All kinds of pipes and outlets made of Polyvinylchlorid or metal mounted on the bridge.
    \end{itemize}
    & 
    \begin{itemize}[leftmargin=*]
        \item The \textit{Drainage} directs water (often contaminated with deicing salt) away from the bridge. 
        \item The draining of water is important for the durability of the bridge. If the water can't drain properly, especially when it's contaminated with deicing salts, the bridge's deterioration is accelerated leading to defects, such as \textit{Spalling}, \textit{Exposed Rebars} or \textit{Rust}
    \end{itemize}
    &
    \includegraphics[height=4.7cm]{SupplMat/img_SupplMat/img_ClassDefs/05010.pdf} % 05010
    \NN

Protective Equipment \linebreak
(PEquipment)
    & 
    \begin{itemize}[leftmargin=*]
        \item Railings, traffic safety features (\eg, steel rail, guide rails, impact attenuation device)
    \end{itemize}
    & 
    \begin{itemize}[leftmargin=*]
        \item Geometric adequacy and structural capacity of the \textit{Protective Equipment} is important with respect to the traffic safety. 
        \item The rail types and installation heights and minimum clearances must be checked.    
        \item Note: Mostly, they are corroded (\textit{Rust}) or deformed due to vehicle impact.
    \end{itemize}
    &
    \includegraphics[height=4.7cm]{SupplMat/img_SupplMat/img_ClassDefs/09195.pdf} % 09195
    \NN
    
Joint Tape \linebreak
(JTape)
    & 
    \begin{itemize}[leftmargin=*]
        \item  All joints that are filled with elastomer or silicon
        \item Note: Originally, \textit{Joint Tape} means an elastomer strap at the end and beginning of relatively small bridges. 
    \end{itemize}
    & 
    \begin{itemize}[leftmargin=*]
        \item \textit{Joint Tapes} compensate longitudinal enlargements due to changes in temperature (like \textit{Expansion Joint}).
        \item Note: A \textit{Joint Tape} is damaged when it's ruptured or twisted. \textit{Joint Tape} is also called Bridge Seal.
    \end{itemize}
    &
    \includegraphics[height=4.7cm]{SupplMat/img_SupplMat/img_ClassDefs/01754.pdf} % 08708 01754 (Silicon) % 03146 (Elastomer) 
    \LL
}



% Background
%     & 
%     \begin{itemize}[leftmargin=*]
%         \item asd
%     \end{itemize}
%     & 
%     \begin{itemize}[leftmargin=*]
%         \item asd
%     \end{itemize}
%     &
%     \includegraphics[height=3.15cm]{img/03752.jpg}
%     \LL


==> SupplMat/8_AddResults.tex <==

%--------------------------------testdev+test---------------------------
\begin{table}[!h]
\begin{center}
\footnotesize
\begin{tabular}{@{}lrrrr@{}}
\toprule
     Class    &   Precision  &  Recall & F1 Score &  \#images \\ \midrule
        Crack &      0.77    &  0.52   &   0.62   &    485 \\
       ACrack &      0.78    &  0.61   &   0.68   &     97 \\
Efflorescence &      0.82    &  0.60   &   0.69   &    460 \\
   Rockpocket &      0.68    &  0.55   &   0.60   &    529 \\
     WConccor &      0.42    &  0.24   &   0.31   &     33 \\
  Hollowareas &      0.84    &  0.77   &   0.81   &    312 \\
     Spalling &      0.80    &  0.76   &   0.78   &   1010 \\
 Restformwork &      0.69    &  0.51   &   0.59   &    251 \\ \midrule
      Wetspot &      0.59    &  0.42   &   0.49   &    298 \\
         Rust &      0.88    &  0.72   &   0.79   &    972 \\
     Graffiti &      0.87    &  0.67   &   0.76   &    235 \\
   Weathering &      0.75    &  0.68   &   0.72   &    916 \\ \midrule
ExposedRebars &      0.80    &  0.59   &   0.68   &    234 \\
      Bearing &      0.85    &  0.82   &   0.83   &    203 \\
       EJoint &      0.74    &  0.67   &   0.70   &     93 \\
     Drainage &      0.88    &  0.54   &   0.67   &    294 \\
   PEquipment &      0.88    &  0.81   &   0.84   &    396 \\
        JTape &      0.75    &  0.58   &   0.66   &    264 \\
%    micro avg &      0.79    &  0.65   &   0.72   &   7082 \\
%    macro avg &      0.77    &  0.61   &   0.68   &   7082 \\
% weighted avg &      0.79    &  0.65   &   0.71   &   7082 \\
%  samples avg &      0.79    &  0.67   &   0.69   &   7082 \\
\bottomrule
\end{tabular}
\caption{Test results for auxiliary head of the best model.} % t
\label{tab:test-results-aux}
\end{center}
\end{table}

%#############################
% Describe classification results on testdev:
\section{Baseline experiments}
\subsection{Additional training informations}
For each of the six combinations of encoder and semantic segmentation architecture, we examined a grid search for the learning rates $1e^{-4}$, $5e^{-4}$, $1e^{-3}$ and $5e^{-3}$ where the best value is chosen based on the validation loss. 
% $0.0005$, $0.0001$, $0.001$ and $0.005$ 

\subsection{Auxiliary multi-label results}
In Table~\ref{tab:test-results-aux} we display additional metrics from the auxiliary head of the best model on the test split. 


\begin{comment}
\begin{table}[h]
\begin{center}
\small
\begin{tabular}{@{}llllllll@{}}
\toprule
        Class & precision &    recall &  f1-score &  support \\  \midrule
        Crack &      0.80  &    0.52 &      0.63 &       239 \\
       ACrack &      0.79  &    0.62 &      0.70 &        48 \\
      Wetspot &      0.61  &    0.41 &      0.49 &       148 \\
Efflorescence &      0.77  &    0.63 &      0.69 &       235 \\
         Rust &      0.87  &    0.79 &      0.83 &       473 \\
   Rockpocket &      0.69  &    0.53 &      0.60 &       266 \\
  Hollowareas &   of   0.83  &    0.73 &      0.78 &       164 \\
     Spalling &      0.79  &    0.77 &      0.78 &       517 \\
     Graffiti &      0.84  &    0.72 &      0.78 &       122 \\
   Weathering &      0.75  &    0.74 &      0.75 &       466 \\
 Restformwork &      0.69  &    0.50 &      0.58 &       133 \\
ExposedRebars &      0.80  &    0.59 &      0.68 &       116 \\
      Bearing &      0.86  &    0.77 &      0.81 &       104 \\
       EJoint &      0.83  &    0.64 &      0.72 &        55 \\
     Drainage &      0.86  &    0.52 &      0.64 &       163 \\
   PEquipment &      0.90  &    0.83 &      0.86 &       199 \\
        JTape &      0.76  &    0.65 &      0.70 &       145 \\
     WConccor &      0.22  &    0.12 &      0.16 &        16 \\  \midrule
    micro avg &      0.79  &    0.67 &      0.73 &      3609 \\
    macro avg &      0.76  &    0.62 &      0.68 &      3609 \\
 weighted avg &      0.79  &    0.67 &      0.72 &      3609 \\
  samples avg &      0.78  &    0.68 &      0.70 &      3609 \\
\bottomrule
\end{tabular}
\caption{--outdated--Test results for best model. {\color{red} Under Construction}}
\label{tab:test-table}
\end{center}
\end{table}


\begin{table}[h]
\begin{center}
\small
\begin{tabular}{@{}llllllll@{}}
\toprule
     Class    &   precision  &  recall & f1-score &  support \\ \midrule
        Crack &      0.81 &      0.54 &      0.65 &       254\\
       ACrack &      0.69 &      0.64 &      0.67 &        42\\
      Wetspot &      0.58 &      0.44 &      0.50 &       144\\
Efflorescence &      0.77 &      0.61 &      0.68 &       206\\
         Rust &      0.88 &      0.75 &      0.81 &       465\\
   Rockpocket &      0.69 &      0.57 &      0.63 &       259\\
  Hollowareas &      0.86 &      0.72 &      0.79 &       155\\
     Spalling &      0.76 &      0.77 &      0.76 &       485\\
     Graffiti &      0.96 &      0.73 &      0.83 &       146\\
   Weathering &      0.69 &      0.75 &      0.72 &       407\\
 Restformwork &      0.78 &      0.53 &      0.63 &       132\\
ExposedRebars &      0.77 &      0.55 &      0.64 &       104\\
      Bearing &      0.94 &      0.73 &      0.82 &       105\\
       EJoint &      0.81 &      0.67 &      0.73 &        51\\
     Drainage &      0.83 &      0.57 &      0.67 &       151\\
   PEquipment &      0.85 &      0.81 &      0.83 &       175\\
        JTape &      0.75 &      0.68 &      0.71 &       128\\
     WConccor &      0.50 &      0.20 &      0.29 &        15\\ \midrule
    micro avg &      0.78 &      0.67 &     0.72 &      3424 \\
    macro avg &      0.77 &      0.63 &     0.69 &      3424 \\
 weighted avg &      0.79 &      0.67 &     0.72 &      3424 \\
  samples avg &      0.77 &      0.69 &     0.70 &      3424 \\ \bottomrule
\end{tabular}
\caption{--outdated--Validation results for best model. {\color{red} Under Construction}}
\label{tab:valid-table}
\end{center}
\end{table}
\end{comment}

%--------------------------------valid---------------------------
\begin{table}[ht]
\begin{center}
\footnotesize
\begin{tabular}{@{}lrrrr@{}}
\toprule
     Class    &   Precision  &  Recall & F1 Score &  Support \\ \midrule
Crack                 &      0.79 &     0.55  &    0.65   &    254 \\
ACrack                &      0.81 &     0.71  &    0.76   &     42 \\
Efflorescence         &      0.83 &     0.58  &    0.68   &    206 \\
Rockpocket            &      0.72 &     0.59  &    0.65   &    259 \\
WConcCor    &      0.50 &     0.07  &    0.12   &     15 \\ 
Hollowareas           &      0.83 &     0.69  &    0.75   &    155 \\
Spalling              &      0.76 &     0.75  &    0.75   &    485 \\
Restformwork          &      0.76 &     0.53  &    0.62   &    132 \\ \midrule
Wetspot              &      0.61 &     0.46  &    0.52   &    144 \\
Rust                  &      0.87 &     0.74  &    0.80   &    465 \\
Graffiti              &      0.93 &     0.72  &    0.81   &    146 \\
Weathering            &      0.73 &     0.72  &    0.73   &    407 \\ \midrule
ExposedRebars        &      0.83 &     0.58  &    0.68   &    104 \\
Bearing               &      0.90 &     0.80  &    0.85   &    105 \\
EJoint       &      0.74 &     0.67  &    0.70   &     51 \\
Drainage              &      0.81 &     0.52  &    0.63   &    151 \\
PEquipment  &      0.87 &     0.82  &    0.84   &    175 \\
JTape            &      0.80 &     0.65  &    0.72   &    128 \\
%    micro avg &      0.79 &     0.66  &    0.72   &   3424 \\
%    macro avg &      0.78 &     0.62  &    0.68   &   3424 \\
% weighted avg &      0.79 &     0.66  &    0.72   &   3424 \\
%  samples avg &      0.78 &     0.68  &    0.70   &   3424 \\
\bottomrule
\end{tabular}
\caption{Validation results for best model.}
\label{tab:test-table}
\end{center}
\end{table}
%--------------------------------valid---------------------------

\begin{comment}
%--------------------------------testdev---------------------------
\begin{table}[h]
\begin{center}
\footnotesize
\begin{tabular}{@{}lrrrr@{}}
\toprule
     Class    &   Precision  &  Recall & F1 Score &  Support \\ \midrule
Crack                 &      0.75    &  0.53   &   0.62   &    239 \\
ACrack       &      0.84    &  0.65   &   0.73   &     48 \\
Efflorescence         &      0.81    &  0.60   &   0.69   &    235 \\
Rockpocket            &      0.67    &  0.53   &   0.59   &    266 \\
WConcCor    &      0.40    &  0.25   &   0.31   &     16 \\
Hollowareas           &      0.82    &  0.74   &   0.78   &    164 \\
Spalling              &      0.81    &  0.77   &   0.79   &    517 \\
Restformwork          &      0.68    &  0.51   &   0.58   &    133 \\ \midrule
Wetspot              &      0.58    &  0.43   &   0.49   &    148 \\
Rust                  &      0.88    &  0.73   &   0.80   &    473 \\
Graffiti              &      0.89    &  0.64   &   0.74   &    122 \\
Weathering            &      0.77    &  0.71   &   0.74   &    466 \\ \midrule
ExposedRebars        &      0.81    &  0.62   &   0.70   &    116 \\
Bearing               &      0.85    &  0.82   &   0.83   &    104 \\
EJoint       &      0.83    &  0.69   &   0.75   &     55 \\
Drainage              &      0.86    &  0.46   &   0.60   &    163 \\
PEquipment &      0.90    &  0.81   &   0.85   &    199 \\
JTape            &      0.79    &  0.60   &   0.68   &    145 \\

%    micro avg &      0.80    &  0.66   &   0.72   &   3609 \\
%    macro avg &      0.77    &  0.62   &   0.68   &   3609 \\
% weighted avg &      0.79    &  0.66   &   0.72   &   3609 \\
%  samples avg &      0.79    &  0.67   &   0.70   &   3609 \\
 \bottomrule
\end{tabular}
\caption{Testdev results for best model.}
\label{tab:testdev-table}
\end{center}
\end{table}
%--------------------------------testdev---------------------------

%--------------------------------test---------------------------
\begin{table}[h]
\begin{center}
\footnotesize
\begin{tabular}{@{}lrrrr@{}}
\toprule
     Class    &   Precision  &  Recall & F1 Score &  Support \\ \midrule
Crack                 &      0.79    &  0.50   &   0.62   &    246 \\
ACrack      &      0.72    &  0.57   &   0.64   &     49 \\
Efflorescence         &      0.83    &  0.59   &   0.69   &    225 \\
Rockpocket            &      0.68    &  0.56   &   0.62   &    263 \\
WConcCor    &      0.44    &  0.24   &   0.31   &     17 \\ %\midrule
Hollowareas           &      0.86    &  0.81   &   0.84   &    148 \\
Spalling              &      0.79    &  0.74   &   0.77   &    493 \\
Restformwork          &      0.70    &  0.51   &   0.59   &    118 \\ \midrule
Wetpot              &      0.60    &  0.41   &   0.49   &    150 \\
Rust                  &      0.88    &  0.72   &   0.79   &    499 \\
Graffiti              &      0.86    &  0.70   &   0.77   &    113 \\
Weathering            &      0.73    &  0.66   &   0.69   &    450 \\ \midrule
ExposedRebars        &      0.79    &  0.55   &   0.65   &    118 \\
Bearing               &      0.84    &  0.82   &   0.83   &     99 \\
EJoint       &      0.63    &  0.63   &   0.63   &     38 \\
Drainage              &      0.90    &  0.63   &   0.74   &    131 \\
PEquipment  &      0.86    &  0.81   &   0.83   &    197 \\
JTape            &      0.71    &  0.55   &   0.62   &    119 \\
%    micro avg &      0.79    &  0.65   &   0.71   &   3473 \\
%    macro avg &      0.76    &  0.61   &   0.67   &   3473 \\
% weighted avg &      0.79    &  0.65   &   0.71   &   3473 \\
%  samples avg &      0.78    &  0.67   &   0.69   &   3473 \\
\bottomrule
\end{tabular}
\caption{Test results for best model.}
\label{tab:test-table}
\end{center}
\end{table}
%--------------------------------test---------------------------
\end{comment}



\begin{comment}
    

\subsection{Qualitative results}
In addition to the qualitative evaluation within the Engineer vs. Machine comparison in the main paper, we show the predictions of the best model on a selection of challenging samples from the test set.  

\begin{figure*}[h]
\begin{center}
\begin{subfigure}[b]{.85\textwidth}
    \includegraphics[height=.33\textwidth]{SupplMat/img_SupplMat/img_ProbClassPreds/05924.pdf}\hfill
    \includegraphics[height=.33\textwidth]{SupplMat/img_SupplMat/img_ProbClassPreds/08940.pdf}\hfill
    \includegraphics[height=.33\textwidth]{SupplMat/img_SupplMat/img_ProbClassPreds/07376.pdf}\hfill
     \caption{Crack.}
   \label{fig:ClassProblems} 
\end{subfigure}
\begin{subfigure}[b]{.85\textwidth}
   \includegraphics[height=.33\textwidth]{SupplMat/img_SupplMat/img_ProbClass/03679.jpg}\hfill
   \caption{Image quality problems: backlight, flash, partial overexposure.}
   \label{fig:ImgQualProb} 
\end{subfigure}
\caption{General problems across the dataset.}
\label{fig:GeneralProblems}
\end{center}
\end{figure*}
\end{comment}
